Motors and Impossible Firing Patterns in the Parallel Chip-Firing Game

The parallel chip-firing game is an automaton on graphs in which vertices "fire" chips to their neighbors when they have enough chips to do so. The game is always periodic, and we concern ourselves with the firing sequences of vertices. We introduce the concepts of motorized parallel chip-firing games and motor vertices, study the effects of motors connected to a tree and show that motorized games can be transformed into ordinary games if the motors' firing sequences occur in some ordinary game. We then characterize exactly which periodic firing patterns can occur in an ordinary game and state some implications of the finding.

==> bellmanFord_sidma.tex <==
\section*{Appendix: The Bellman-Ford Algorithm} \label{bfAlg}
The following Python program below constructs $\G$ from Section~\ref{binSeq}
and shows it has no negative cycles. For a more detailed exposition of the
Bellman-Ford algorithm and a proof of its validity, see~\cite{bellmanford}.

\bigskip
\footnotesize
\verbatiminput{bellmanFord.py}
\normalsize

